An Improved Dictatorship Test with Perfect Completeness

A Boolean function $f:\{0,1\}^n\rightarrow \{0,1\}$ is called a dictator if it depends on exactly one variable i.e $f(x_1, x_2, \ldots, x_n) = x_i$ for some $i\in [n]$. In this work, we study a $k$-query dictatorship test. Dictatorship tests are central in proving many hardness results for constraint satisfaction problems. The dictatorship test is said to have {\em perfect completeness} if it accepts any dictator function. The {\em soundness} of a test is the maximum probability with which it accepts any function far from a dictator. Our main result is a $k$-query dictatorship test with perfect completeness and soundness $ \frac{2k + 1}{2^k}$, where $k$ is of the form $2^t -1$ for any integer $t > 2$. This improves upon the result of \cite{TY15} which gave a dictatorship test with soundness $ \frac{2k + 3}{2^k}$.

==> prelims.tex <==
\iffalse
{
\section{Basics (Advanced topics)}


A probability space is denoted by $\rho(\Omega; p_1, p_2,\ldots, p_l)$ where $\Omega = \{\omega_1,\omega_2,\ldots, \omega_l\}$ and all $p_i>0$ denotes $\Pr_{x\sim \rho}[x=\omega_i]$. We are interested in functions $f :\Omega^n \rightarrow \R$. We will denote a vector of length $n$ by a bold face letter (such as $\v{x}, \v{\sigma}$) and the $ith$ coordinate of a vector by simply the same letter with $i$ as a subscript (such as $x_i, \sigma_i$). 

\subsection{Fourier Analysis}
Let us consider the simplest case when $n=1$. In this case, a function $f:\Omega \rightarrow \R$ is just a vector of length $l$. We define an inner product on this space of functions as  
$$\langle f, g\rangle = \E_{x\sim \rho}[f(x)\cdot g(x)] :=\sum_{i=1}^{l}[p_i f(\omega_i)g(\omega_i)].$$

Let $\chi_0, \chi_1,\ldots, \chi_{l-1} : \Omega \rightarrow \R$ be a set of functions (called as $characters$) with the following property:
\begin{enumerate}
    \item $\chi_0$ is a constant $1$ function.
    \item $\langle \chi_i, \chi_i\rangle = 1$ for all $0\leq i\leq l-1$.
    \item $\langle \chi_i, \chi_j\rangle = 0$ for all $i\neq j$.
\end{enumerate}


\begin{fact}
There exists $\chi_0, \chi_1, \ldots, \chi_{l-1}$ with the above properties.
\end{fact}

\begin{fact}
Every function $f : \Omega \rightarrow \R$ can be written as $f = \sum_{i=0}^{l-1} \alpha_i \chi_i$ and is called a fourier expansion of $f$.
\end{fact}

There characters we defined can be used to define characters for space of functions $f : \Omega^n \rightarrow \R$. On this space, we will have a character for every $\v{\sigma} \in [l-1]^n$, denoted by $\chi_{\v{\sigma}} : \Omega^n \rightarrow \R$, defined as:

$$ \chi_{\v{\sigma}} (\v{x}) = \prod_{i=1}^n \chi_{\sigma_i}(x_i).$$

\begin{fact}
$\chi_{\v{\sigma}}$ form a basis for functions $f:\Omega^n \rightarrow \R$ i.e every such function $f$ can be written as 
$$ f = \sum_{\v{\sigma}\in [l-1]^n} \hat{f}(\v{\sigma}) \chi_{\v{\sigma}}.$$
where $\hat{f}(\v{\sigma})$ are called fourier coefficients of $f$.
\end{fact}

We define the size of a fourier coefficient $\hat{f}({\v{\sigma}})$ as the number of non-zero elements in $\v{\sigma}$.


\begin{definition}[Efron-Stein decomposition]
Let $\rho(\Omega; p_1, p_2,\ldots, p_l)$ be a probability space. Every function $f: \Omega^n \rightarrow \R$ can be decomposed into sum of $2^n$ functions i.e. $f = \sum_{S\subseteq [n]} f_S$, such that
$\langle f_S, f_T\rangle = 0$ if $S\neq T$.
\end{definition}

In terms of fourier decomposition above, $f_S$ is precisely $\mathop{\sum}_{\v{\sigma} | \mathtt{supp}(\v{\sigma}) = S} \hat{f}(\v{\sigma})\chi_{\v{\sigma}}$.

\subsection{Correlated spaces}



Let $\Omega_1\times \Omega_2$ be two correlated spaces and $\cald$ denotes the joint distribution. Let $\mu_1$ and $\mu_2$ denote the marginal of $\cald$ on space $\Omega_1$ and $\Omega_2$ respectively. Let $|\Omega_1| = L$ and $|\Omega_2| = M$. The correlated space $\rho(\Omega_1\times \Omega_2; \cald)$ can be represented as a bipartite graph on $(\Omega_1, \Omega_2)$ where $x\in \Omega_1$ is connected to $y\in \Omega_2$ iff $\cald(x,y) > 0$. We say that the correlated spaces is $connected$ if this underlying graph is connected. 

Let $f:\Omega_1 ^n \rightarrow \R$ and $g:\Omega_2^n \rightarrow \R$ are two functions. We are interested in bounding expression of type:

\begin{equation}
\label{eq:inner_prod}
 \mathop{\E}_{(\v{x},\v{y}) \sim \cald^{\otimes n}} [f(\v{x}) \cdot g(\v{y})]
\end{equation}
where $\cald^{\otimes n}$ denotes a distribution on $\Omega_1^n\times \Omega_2^n$ sampled independently for each coordinate w.r.t $\cald$. We will denote the characters on space of functions on $\Omega_1^n$  by $\chi_{\v{\sigma}}$ and characters on space of functions on $\Omega_2^n$ by $\psi_{\v{\tau}}$.

\begin{definition}[Beckner Operator]
Let $\rho(\Omega; p_1, p_2,\ldots, p_l)$ be a probability space. For $\gamma\in [0,1]$ the beckner operator, denoted by $T_{1-\gamma}$, applied on function $f: \Omega^n \rightarrow \R$ is another function from the same space, $T_{1-\gamma}f : \Omega^n
\rightarrow \R$, defined by
$$ T_{1-\gamma}f(\v{x}) = \mathop{\E}_{\v{y}\sim N_\gamma(\v{x})}[f(\v{y})]$$
where $N_\gamma(\v{x})$ is a distribution on $\Omega^n$ such that, independently for each $i\in [n]$ $y_i=x_i$ w.p $1-\gamma$ and w.p $\gamma$ $y_i$ is resampled from $\rho$.
\end{definition}

The following lemma says that if the correlated spaces is connected then in order to bound expression (\ref{eq:inner_prod}), it is enough to consider the {\em low degree part} of $f$ and $g$. 

\begin{lemma}
\label{lemma:low_degree}
Let $\rho(\Omega_1\times \Omega_2;\cald)$ be correlated spaces which is connected. Let $f: \Omega_1^n \rightarrow [-1,1]$ and $g:\Omega_2^n \rightarrow [-1,1]$. Then for all $\epsilon> 0$ there exists $\gamma(\epsilon, \cald)>0$ such that
$$ \left| \mathop{\E}_{(\v{x},\v{y}) \sim \cald^{\otimes n}} [f(\v{x}) \cdot g(\v{y})] - \mathop{\E}_{(\v{x},\v{y}) \sim \cald^{\otimes n}} [T_{1-\gamma}f(\v{x}) \cdot T_{1-\gamma}g(\v{y})]\right| \leq \epsilon$$
\end{lemma}

Before proving the above lemma, let us understand the case when $n=1$ and $f$ and $g$ are character functions. In this case, we would like to bound $\E_{(x,y)\sim \cald}[\chi_i(x)\psi)j(y)]$. Clearly, when both $i=j=0$ then the expression evaluates to $1$. The following claims shows that in all the remaining cases, it is strictly less than $1$. This fact will be useful in proving the lemma.

\begin{claim} For correlated spaces $\rho(\Omega_1\times \Omega_2, \cald)$ where $\cald$ is connected, unless $i=j=0$, 
$$\mathop{\E}_{(x,y)\sim \cald}[\chi_i(x)\psi_j(y)] < 1$$
\end{claim}
\begin{proof}

\begin{align}
    \mathop{\E}_{(x,y)\sim \cald} [\chi_i(x)\psi_j(y)] & = \mathop{\E}_{x}[\chi_i(x) \mathop{\E}_{y}[\psi_j(y) | x]] \nonumber\\
    & \leq \sqrt{\mathop{\E}_{x}[\chi_i(x)^2]} \sqrt{\mathop{\E}_{x}[ \mathop{\E}_{y}[\psi_j(y) | x]^2]}\nonumber\\
    & = \sqrt{\mathop{\E}_{x}[ \mathop{\E}_{y}[\psi_j(y) | x]^2]}\nonumber\\
    &\leq \sqrt{\mathop{\E}_{x}[ \mathop{\E}_{y}[\psi_j(y)^2 | x]]}\label{eq:CS}\\
    &= \sqrt{\mathop{\E}_{y}[ \mathop{\E}_{x}[\psi_j(y)^2 | x]]}\nonumber\\
    &= \sqrt{\mathop{\E}_{y}[\psi_j(y)^2 ]} = 1\nonumber
\end{align}
For any fixed $x\in \Omega_1$, if for all $y\in \Omega_2$ such that $\cald(x,y)>0$, we have $\psi_j(y)$ are all equal then only $(\ref{eq:CS})$ becomes equality. Thus, a necessary condition for  the expression to become $1$ is - for all $x\in \Omega_1$, all its neighbors $y$ get the same value $\psi_j(y)$. If the graph is connected then this condition is never going to satisfy if $\psi_j$ is a non trivial characters. This proves the claim.
\end{proof}

\paragraph{Proof of Lemma~\ref{lemma:low_degree}}: Before beginning the proof, let us analyze the contribution of {\em high degree} terms in the expectation:
$$\mathop{\E}_{(\v{x},\v{y}) \sim \cald^{\otimes n}} [f(\v{x}) \cdot g(\v{y})] = \mathop{\E}_{(\v{x},\v{y}) \sim \cald^{\otimes n}} [\sum_{S\subseteq [n]} f_S\cdot \sum_{T\subseteq [n]} g_T] = \sum_{S\subseteq [n]} \mathop{\E}_{(\v{x},\v{y}) \sim \cald^{\otimes n}}[f_S g_S]$$ 
}
\fi
